SecRepoBench: Benchmarking Code Agents for Secure Code Completion in Real-World Repositories

This paper introduces SecRepoBench, a benchmark to evaluate code agents on secure code completion in real-world repositories. SecRepoBench has 318 code completion tasks in 27 C/C++ repositories, covering 15 CWEs. We evaluate 29 standalone LLMs and 15 code agents across 3 state-of-the-art agent frameworks using our benchmark. We find that state-of-the-art LLMs struggle with generating correct and secure code completions. However, code agents significantly outperform standalone LLMs. We show that SecRepoBench is more difficult than the prior state-of-the-art benchmark. Finally, our comprehensive analysis provides insights into potential directions for enhancing the ability of code agents to write correct and secure code in real-world repositories.

==> tab/sec.tex <==
\begin{table*}[t!]
\centering
\small
\begin{tabular}{@{}l
                      S[table-format=2.1, table-space-text-post=\%]
                      S[table-format=2.1, table-space-text-post=\%]
                      S[table-format=2.1, table-space-text-post=\%]
                      S[table-format=2.1, table-space-text-post=\%]
                      S[table-format=2.1, table-space-text-post=\%]
                      S[table-format=2.1, table-space-text-post=\%]@{}}
        \toprule
                               & \multicolumn{2}{c}{\textbf{sec-generic}} & \multicolumn{2}{c}{\textbf{sec-specific}} & \multicolumn{2}{c}{\textbf{security-policy}} \\
        \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7}
                               & \textbf{\benchmark}  & \textbf{\SecCodePLT}  & \textbf{\benchmark}  & \textbf{\SecCodePLT}  & \textbf{\benchmark}  & \textbf{\SecCodePLT}  \\
        \textbf{Model}         & \textbf{(\%)}          & \textbf{(\%)}        & \textbf{(\%)}          & \textbf{(\%)}        & \textbf{(\%)}          & \textbf{(\%)}        \\
        \midrule
        \claudeSonnettThreeFive{}     & -0.9 & -0.4 & 0.0  & 0.0  & 2.2  & 8.1  \\
        \claudeThreeHaiku{}           & -0.3 & 0.0  & -0.3 & 0.0  & 0.3  & 14.5 \\
        \deepseekVTwoLite{}           & 2.2  & 8.2  & -1.6 & 3.3  & 0.9  & 22.0 \\
        \geminiOneFiveFlash{}         & 0.0  & 5.0  & 1.3  & 5.1  & 1.9  & 27.4 \\
        \geminiOneFivePro{}           & 0.0  & 3.3  & -3.1 & 5.5  & 2.8  & 12.6 \\
        \gptFourOOld{}                & 4.1  & 3.8  & -0.3 & 13.2 & 4.1  & 14.1 \\
        \gptFourOmini{}               & -0.3 & -3.7 & 1.0  & -4.4 & 2.8  & 12.3 \\
        \llamaThreeSeventyB{}         & 0.0  & 30.0 & -0.6 & 7.8  & 1.6  & 36.7 \\
        \llamatTreeEightB{}           & 0.3  & 1.2  & -1.6 & 1.2  & -0.6 & 9.6  \\
        \mistralNemo{}                & -0.6 & 1.6  & 2.5  & 11.9 & 0.3  & 32.4 \\
        \midrule
        \textbf{Average}            & 0.4  & 4.9  & -0.3 & 4.4  & 1.6  & 19.0 \\
        \bottomrule
    \end{tabular}
    \vspace{5pt}
\caption{Changes in \secpassone{} using the prompt engineering methods (sec-generic, sec-specific, and security-policy) compared to using \systemPrompt{} prompt for \benchmark{} and \SecCodePLT. On average, security-policy prompt increases the \secpassone{} on \SecCodePLT by 19\%, but only by 1.6\% on \benchmark{}.}
\label{prompt engineering benchmark comparison}
\end{table*}
